Successive Refinement of Images with Deep Joint Source-Channel Coding

We introduce deep learning based communication methods for successive refinement of images over wireless channels. We present three different strategies for progressive image transmission with deep JSCC, with different complexity-performance trade-offs, all based on convolutional autoencoders. Numerical results show that deep JSCC not only provides graceful degradation with channel signal-to-noise ratio (SNR) and improved performance in low SNR and low bandwidth regimes compared to state-of-the-art digital communication techniques, but can also successfully learn a layered representation, achieving performance close to a single-layer scheme. These results suggest that natural images encoded with deep JSCC over Gaussian channels are almost successively refinable.

==> figures/model_multiple_decoders.tex <==
% \documentclass[10pt, conference]{IEEEtran}
% \usepackage{lmodern}
% \usepackage{tikz}
% \usepackage{bm}
% \usetikzlibrary{shapes.geometric, arrows, positioning, fit}


 \tikzstyle{txt} = [text centered]
 \tikzstyle{box} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1.5cm, text width=2.5cm, text centered, draw=black]
 \tikzstyle{bbox} = [rectangle, thick, minimum width=1.5cm, minimum height=1cm, text width=1.5cm, text centered, draw=black]
 \tikzstyle{arrow} = [thick,->,>=stealth]
 \tikzstyle{fitted} = [draw=gray, thick, dotted, inner sep=0.75em]

% \begin{document}


\begin{tikzpicture}[node distance=2.3cm]

\node (x) [txt, font=\fontsize{14}{0}\selectfont] {$\bm{x}$};
\node (encoder) [box, right of=x, font=\fontsize{12}{12}\selectfont] {Encoder \\ ($f_{\bm{\theta}}$)};
\node (z) [txt, right of=encoder, xshift=0.5cm, font=\fontsize{14}{0}\selectfont] { };
% transmission 1
\node (channel1) [bbox, above right of=z,  font=\fontsize{12}{12}\selectfont, xshift=0.5cm, yshift=-0.5cm] {channel};
% \node (zhat1) [txt, right of=channel1, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
\node (decoder1) [box, right of=channel1, xshift=1.5cm,  font=\fontsize{12}{12}\selectfont] {Decoder1\\($g_{\bm{\phi_1}}$)};
\node (xhat1) [txt, right of=decoder1,font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_1}$};
\node (baselayer) [fitted, fit=(channel1) (decoder1)] {};
\node at (baselayer.north) [above, inner sep=1mm] {Base Layer};

% transmission 2
\node (channel2) [bbox, below right of=z,  font=\fontsize{12}{12}\selectfont, xshift=0.5cm, yshift=0.5cm] {channel};
% \node (zhat2) [txt, right of=channel2, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
\node (decoder2) [box, right of=channel2, xshift=1.5cm,  font=\fontsize{12}{12}\selectfont] {Decoder2\\($g_{\bm{\phi_2}}$)};
\node (xhat2) [txt, right of=decoder2,font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_2}$};
\node (reflayer) [fitted, fit=(channel2) (decoder2)] {};
\node at (reflayer.south) [below, inner sep=1mm] {Refinement Layer};

% \node (rx) [fitted, fit=(sdecoder) (demodulator)] {};
% \node at (rx.north) [above, inner sep=3mm] {Receiver};

\draw [arrow] (x) -- (encoder);
% base layer
\draw [arrow] (encoder.east) 
-- node[above,font=\fontsize{14}{0}\selectfont] {$\bm{z}$} ++(1, 0) |- node[above right,font=\fontsize{14}{0}\selectfont] {$\bm{z_1}$}  (channel1.west);
\draw [arrow] (channel1) -- node[above,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_1$} (decoder1);
\draw [arrow] (decoder1) -- (xhat1);
% refinement layer
\draw [arrow] (encoder.east) 
-- ++(1, 0) |- node[below right,font=\fontsize{14}{0}\selectfont] {$\bm{z_2}$}  (channel2.west);
\draw [arrow] (channel2.350) -- node[above left,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_2$} (decoder2.187);
\draw [arrow] (channel1.east) -- ++(0.75, 0) |- (decoder2.165);
\draw [arrow] (decoder2) -- (xhat2);

%\draw [arrow] (encoder.east) -- node[above,font=\fontsize{14}{0}\selectfont] {$\bm{z}$} ++(0.0, 1.0) -| (channel1);
% \draw [arrow] (channel1.south) -- ++(0,-1.0) -- node[below,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}$}(demodulator);
% \draw [arrow] (demodulator) --  (cdecoder);
% \draw [arrow] (cdecoder) --  (sdecoder);
% \draw [arrow] (sdecoder) --(xhat);


\end{tikzpicture}


% \end{document}

==> figures/model_resnet.tex <==
% \documentclass[10pt, conference]{IEEEtran}
% \usepackage{lmodern}
% \usepackage{tikz}
% \usepackage{bm}
% \usetikzlibrary{shapes.geometric, arrows, positioning, fit}


 \tikzstyle{txt} = [text centered]
 \tikzstyle{box} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1.5cm, text width=2.5cm, text centered, draw=black]
 \tikzstyle{bbox} = [rectangle, thick, minimum width=1.5cm, minimum height=1cm, text width=1.5cm, text centered, draw=black]
 \tikzstyle{arrow} = [thick,->,>=stealth]
 \tikzstyle{fitted} = [draw=gray, thick, dotted, inner sep=0.75em]
 \tikzstyle{sum} = [draw, circle]

% \begin{document}

\begin{tikzpicture}[node distance=2.3cm]

% transmission 1
\node (x1) [txt, font=\fontsize{14}{0}\selectfont] {$\bm{x}$};
\node (encoder1) [box, right of=x1, xshift=0.5cm, font=\fontsize{12}{12}\selectfont] {Encoder \\ ($f_{\bm{\theta}_1}$)};
% \node (z) [txt, right of=encoder, xshift=0.5cm, font=\fontsize{14}{0}\selectfont] { };
\node (channel1) [bbox, right of=encoder1, xshift=1cm, font=\fontsize{12}{12}\selectfont, xshift=0.5cm] {channel};
% \node (zhat1) [txt, right of=channel1, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
\node (decoder1) [box, right of=channel1, xshift=1.5cm,  font=\fontsize{12}{12}\selectfont] {Decoder1\\($g_{\bm{\phi_1}}$)};
\node (xhat1) [txt, right of=decoder1,font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_1}$};
\node (baselayer) [fitted, fit=(channel1) (decoder1)] {};
\node at (baselayer.north) [above, inner sep=1mm] {Base Layer};

% transmission 2
\node (x2) [txt, below of=x1, font=\fontsize{14}{0}\selectfont] {$\bm{x-\hat{x}'_1}$};
\node (encoder2) [box, right of=x2, xshift=0.5cm, font=\fontsize{12}{12}\selectfont] {Encoder \\ ($f_{\bm{\theta}_2}$)};
\node (channel2) [bbox, right of=encoder2, xshift=1cm, font=\fontsize{12}{12}\selectfont, xshift=0.5cm] {channel};
% \node (zhat2) [txt, right of=channel2, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
\node (decoder2) [box, right of=channel2, xshift=1.5cm, font=\fontsize{12}{12}\selectfont] {Decoder2\\($g_{\bm{\phi_2}}$)};
\node (adder) [sum, right of=decoder2] {\Large$+$};
\node (xhat2) [txt, right of=adder, xshift=-0.8cm, font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_2}$};
\node (reflayer) [fitted, fit=(channel2) (adder)] {};
\node at (reflayer.south) [below, inner sep=1mm] {Refinement Layer};

% \node (rx) [fitted, fit=(sdecoder) (demodulator)] {};
% \node at (rx.north) [above, inner sep=3mm] {Receiver};

% base layer
\draw [arrow] (x1) -- (encoder1);
\draw [arrow] (encoder1) -- node[above,font=\fontsize{14}{0}\selectfont] {$\bm{z_1}$} (channel1);
\draw [arrow] (channel1) -- node[above,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_1$} (decoder1);
\draw [arrow] (decoder1) -- (xhat1);
% refinement layer
\draw [arrow] (x2) -- (encoder2);
\draw [arrow] (encoder2) -- node[above,font=\fontsize{14}{0}\selectfont] {$\bm{z_1}$} (channel2);
\draw [arrow] (channel2) -- node[above,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_2$} (decoder2);
\draw [arrow] (decoder2) -- (adder);
\draw [arrow] (xhat1) -- (adder);
\draw [arrow] (adder) -- (xhat2);
% \draw [arrow] (encoder.east) 
% -- ++(1, 0) |- node[below right,font=\fontsize{14}{0}\selectfont] {$\bm{z_2}$}  (channel2.west);
% \draw [arrow] (channel2.350) -- node[above left,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_2$} (decoder2.187);
% \draw [arrow] (channel1.east) -- ++(0.75, 0) |- (decoder2.165);
% \draw [arrow] (decoder2) -- (xhat2);


\end{tikzpicture}

% \end{document}

==> figures/model_single_decoder.tex <==
% \documentclass[10pt, conference]{IEEEtran}
% \usepackage{lmodern}
% \usepackage{tikz}
% \usepackage{bm}
% \usetikzlibrary{shapes.geometric, arrows, positioning, fit}


 \tikzstyle{txt} = [text centered]
 \tikzstyle{box} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1.5cm, text width=2.5cm, text centered, draw=black]
 \tikzstyle{bbox} = [rectangle, thick, minimum width=1.5cm, minimum height=1cm, text width=1.5cm, text centered, draw=black]
 \tikzstyle{arrow} = [thick,->,>=stealth]
 \tikzstyle{fitted} = [draw=gray, thick, dotted, inner sep=0.75em]

% \begin{document}


\begin{tikzpicture}[node distance=2.3cm]

\node (x) [txt, font=\fontsize{14}{0}\selectfont] {$\bm{x}$};
\node (encoder) [box, right of=x, font=\fontsize{12}{12}\selectfont] {Encoder \\ ($f_{\bm{\theta}}$)};
\node (z) [txt, right of=encoder, xshift=0.5cm, font=\fontsize{14}{0}\selectfont] { };
% transmission 1
\node (channel1) [bbox, above right of=z,  font=\fontsize{12}{12}\selectfont, xshift=0.5cm, yshift=-0.5cm] {channel};
% \node (zhat1) [txt, right of=channel1, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
% \node (decoder1) [box, right of=channel1, xshift=1.5cm,  font=\fontsize{12}{12}\selectfont] {Decoder1\\($g_{\bm{\phi_1}}$)};
\node (decoder) [box, below right of=channel1, xshift=2.5cm, yshift=0.5cm, font=\fontsize{12}{12}\selectfont] {Decoder\\($g_{\bm{\phi}}$)};
\node (xhat1) [txt, above right of=decoder, xshift=1cm, font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_1}$};
% \node (baselayer) [fitted, fit=(channel1) (decoder1)] {};
% \node at (baselayer.north) [above, inner sep=1mm] {Base Layer};

% transmission 2
\node (channel2) [bbox, below right of=z,  font=\fontsize{12}{12}\selectfont, xshift=0.5cm, yshift=0.5cm] {channel};
% \node (zhat2) [txt, right of=channel2, font=\fontsize{14}{0}\selectfont,xshift=0.5cm] {};
% \node (decoder2) [box, right of=channel2, xshift=1.5cm,  font=\fontsize{12}{12}\selectfont] {Decoder2\\($g_{\bm{\phi_2}}$)};
\node (xhat2) [txt, below right of=decoder, xshift=1cm, font=\fontsize{14}{0}\selectfont] {$\bm{\hat{x}_2}$};
% \node (reflayer) [fitted, fit=(channel2) (decoder2)] {};
% \node at (reflayer.south) [below, inner sep=1mm] {Refinement Layer};

% \node (rx) [fitted, fit=(sdecoder) (demodulator)] {};
% \node at (rx.north) [above, inner sep=3mm] {Receiver};



\draw [arrow] (x) -- (encoder);
% % base layer
\draw [arrow] (encoder.east) 
-- node[above,font=\fontsize{14}{0}\selectfont] {$\bm{z}$} ++(1, 0) |- node[above right,font=\fontsize{14}{0}\selectfont] {$\bm{z_1}$}  (channel1.west);
\draw [arrow] (channel1) -- node[above,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_1$} ++(2,0) |- (decoder);
\draw [arrow] (decoder) -| (xhat1);
% % refinement layer
\draw [arrow] (encoder.east) 
-- ++(1, 0) |- node[below right,font=\fontsize{14}{0}\selectfont] {$\bm{z_2}$}  (channel2.west);
\draw [arrow] (channel2) -- node[below,font=\fontsize{14}{0}\selectfont] {$\hat{\bm{z}}_2$} ++(2,0) |- (decoder);
\draw [arrow] (decoder) -| (xhat2);


\end{tikzpicture}


% \end{document}
